FABind+: Enhancing Molecular Docking through Improved Pocket Prediction and Pose Generation

Molecular docking is a pivotal process in drug discovery. While traditional techniques rely on extensive sampling and simulation governed by physical principles, these methods are often slow and costly. The advent of deep learning-based approaches has shown significant promise, offering increases in both accuracy and efficiency. Building upon the foundational work of FABind, a model designed with a focus on speed and accuracy, we present FABind+, an enhanced iteration that largely boosts the performance of its predecessor. We identify pocket prediction as a critical bottleneck in molecular docking and propose a novel methodology that significantly refines pocket prediction, thereby streamlining the docking process. Furthermore, we introduce modifications to the docking module to enhance its pose generation capabilities. In an effort to bridge the gap with conventional sampling/generative methods, we incorporate a simple yet effective sampling technique coupled with a confidence model, requiring only minor adjustments to the regression framework of FABind. Experimental results and analysis reveal that FABind+ remarkably outperforms the original FABind, achieves competitive state-of-the-art performance, and delivers insightful modeling strategies. This demonstrates FABind+ represents a substantial step forward in molecular docking and drug discovery. Our code is in https://github.com/QizhiPei/FABind.

==> chap/9_limitation.tex <==
\section{Limitation}
\label{supp:limitation}
There are also some clear limitations for \method{}. 
While \method{} achieves state-of-the-art results among open-source molecular docking methods, its docking performance remains inferior to that of AlphaFold 3~\cite{abramson2024af3} in a large margin, indicating there is a substantial room for improvement. Additionally, \method{} is currently only limited to blind docking scenarios where the protein is rigidly bound and cannot yet handle flexible docking, which is a more realistic setting.
